AONN-2: An adjoint-oriented neural network method for PDE-constrained shape optimization

Shape optimization has been playing an important role in a large variety of engineering applications. Existing shape optimization methods are generally mesh-dependent and therefore encounter challenges due to mesh deformation. To overcome this limitation, we present a new adjoint-oriented neural network method, AONN-2, for PDE-constrained shape optimization problems. This method extends the capabilities of the original AONN method [1], which is developed for efficiently solving parametric optimal control problems. AONN-2 inherits the direct-adjoint looping (DAL) framework for computing the extremum of an objective functional and the neural network methods for solving complicated PDEs from AONN. Furthermore, AONN-2 expands the application scope to shape optimization by taking advantage of the shape derivatives to optimize the shape represented by discrete boundary points. AONN-2 is a fully mesh-free shape optimization approach, naturally sidestepping issues related to mesh deformation, with no need for maintaining mesh quality and additional mesh corrections. A series of experimental results are presented, highlighting the flexibility, robustness, and accuracy of AONN-2.

==> Research_Highlights.tex <==
1. A new adjoint-oriented neural network method, AONN-2, is proposed for solving PDE-constrained shape optimization problems.

2. AONN-2 inherits the advantages of AONN, which integrates the classical direct-adjoint looping (DAL) framework for optimizing objective functional and the emerging neural network methods for solving PDEs.

3. AONN-2 takes advantage of shape derivative to optimize the shape represented by the shape representing points on the boundary.

4. AONN-2 is completely mesh-free that naturally avoids the difficulties in mesh quality assurance and mesh correction.

5. AONN-2 is superior to the widely-used mesh dependent shape optimization toolbox 'Fireshape' in terms of accuracy, flexibility and robustness.







% It is a completely mesh-free method that naturally avoids the difficulties in mesh quality assurance and mesh correction from the traditional mesh dependent shape optimization method.

% 2. AONN-2 extends AONN to shape optimization problem by taking advantage of shape derivative to optimize the shape represented by discrete boundary points. It inherits the advantages of AONN, which integrates the classical direct-adjoint looping (DAL) framework for optimizing objective functional and the emerging neural network methods for solving PDEs.

% 3. In the numerical experiments about shape optimization problems constrained by the Poisson, Stokes, and Navier-Stokes equations, AONN-2 has demonstrated its mesh-free advantage with showing superior performance in accuracy, flexibility and robustness compared with the widely-used mesh dependent shape optimization toolbox 'Fireshape'.



% 1. In AONN-2, a new adjoint-oriented neural network method is proposed for PDE-constrained shape optimization, which consists of a looping of five steps: solving the state equation (state step), solving the adjoint equation (adjoint step), solving the regularization equation (regularization step), updating the shape representing points (update step), and resampling the collocation points (resample step).

% 2. AONN-2 inherits the advantages of AONN, which integrates the classical direct-adjoint looping (DAL) framework for optimizing objective functional and the emerging neural network methods for solving complicated PDEs.

% 3. We extend the application of AONN to shape optimization problem by taking advantage of shape derivative to optimize the shape represented by discrete boundary points.

% 4. The flexibility, robustness, and accuracy of AONN-2 are demonstrated with shape optimization problems constrained by the Poisson, Stokes, and Navier-Stokes equations, showcasing its mesh-free advantages and superior performance compared to the widely-used shape optimization toolbox, Fireshape.




==> Significance_and_Novelty.tex <==


% In this manuscript, we propose an adjoint-oriented neural network method for PDE-constrained shape optimization (AONN-2). The significance and novelty of this work are as follows. It expands AONN to shape optimization by taking advantage of shape derivative to optimize the shape represented by shape representing points. AONN-2 is a compeletly mesh-free shape optimization method that naturally avoids the issues caused by mesh dependency. It inherits the advantages from AONN, which integrates the classical direct-adjoint looping (DAL) framework for computing the extremum of an objective functional and the emerging mesh-free neural network methods for solving PDEs. Experimental results demonstrate that the proposed AONN-2 method outperforms the traditional mesh-dependent shape optimization method in accuracy, flexibility and robustness.


In this manuscript, we propose an adjoint-oriented neural network method for PDE-constrained shape optimization (AONN-2). The significance and novelty of this work are as follows. AONN-2 is a compeletly mesh-free shape optimization method that naturally avoids the issues caused by mesh dependency. It inherits the advantages from AONN, which integrates the classical direct-adjoint looping (DAL) framework for computing the extremum of an objective functional and the emerging neural network methods for solving complicated PDEs. Additionally, AONN-2 expands the application of AONN to shape optimization by taking advantage of shape derivative to optimize the shape represented by shape representing points. Experimental results demonstrate that the proposed AONN-2 method outperforms the traditional mesh-dependent shape optimization method in accuracy, flexibility and robustness.


